SaGe: Preemptive Query Execution for High Data Availability on the Web

Semantic Web applications require querying available RDF Data with high performance and reliability. However, ensuring both data availability and performant SPARQL query execution in the context of public SPARQL servers are challenging problems. Queries could have arbitrary execution time and unknown arrival rates. In this paper, we propose SaGe, a preemptive server-side SPARQL query engine. SaGe relies on a preemptable physical query execution plan and preemptable physical operators. SaGe stops query execution after a given slice of time, saves the state of the plan and sends the saved plan back to the client with retrieved results. Later, the client can continue the query execution by resubmitting the saved plan to the server. By ensuring a fair query execution, SaGe maintains server availability and provides high query throughput. Experimental results demonstrate that SaGe outperforms the state of the art SPARQL query engines in terms of query throughput, query timeout and answer completeness.

==> figures/bgp_evaluation.tex <==
\begin{algorithm}
  \SetAlgoVlined
  \SetKwInput{KwInit}{Init}
  \SetKwFor{Foreach}{for each}{do}{endfor}
  \SetKwProg{Fn}{Function}{\string:}{}
  \SetKwProg{Proc}{Procedure}{\string:}{}
  \SetKwProg{Event}{Event}{\string:}{}
  \SetKwComment{tcp}{}{}%
  \SetKwComment{tcc}{// }{}%

  \DontPrintSemicolon
  \SetInd{0.55em}{0.55em}
  \caption{BGP evaluation}\label{algo:query_evaluation}

  \KwIn{
    $BGP = \{ tp_1, \dots, tp_n \}$: set of triples patterns,
    $\mathcal{D}$: RDF dataset,
    $P$: serialized query execution plan,
    $q$: quota in time
  }

  \Fn{EvaluateRequest(BGP, $\mathcal{D}$, P, q)}{
    \eIf{$P \neq nil$}{
      $I \leftarrow Deserialize(P)$ \; \label{algo:line:deserialize_plan}
    }{
      $I \leftarrow BuildQueryPlan(BGP, \mathcal{D})$ \; \label{algo:line:build_plan}
    }

    \tcc{Evaluate the query execution plan under the time quota}
    $\mathcal{V} \leftarrow \emptyset$ \;
    \textbf{StartTimer} invoke $I.Close()$ after $q$ is exceeded \; \label{algo:line:start_timer}
    $v \leftarrow I.Next()$ \;
    \While{\textbf{not} $I.IsDone()$ \textbf{and} $v \neq nil$}{ \label{algo:line:plan_evaluation}
      $\mathcal{V} \leftarrow \mathcal{V} \medcup \{ v \}$ \;
      $v \leftarrow I.Next()$ \; \label{algo:line:advance_plan}
    }

    % \tcc{access index to get real values, then do joins}
    % $\mu \leftarrow \emptyset$\;
    % \For{$tp_i \in triples$}{
    %   $\Omega \leftarrow \{ t | \forall v_j \in \mathcal{V}, t = values(v_j, tp_i) \}$ \;
    %   $\mu \leftarrow \mu \bowtie \pi_{vars(tp_i)}\Omega $\;
    % }

    \tcc{Save execution plan for the next evaluation step}
    $P' \leftarrow nil$ \;
    \If{\textbf{not} $I.IsDone()$}{
      $P' \leftarrow Serialize(I)$ \; \label{algo:line:serialize_plan}
    }
    \Return $\langle \mathcal{V}, P' \rangle$ \;
  }
  \BlankLine
\end{algorithm}


==> figures/bgp_iteratorOld.tex <==
\begin{algorithm}[t]
  \SetAlgoVlined
  \SetKwInput{Data}{Require}
  \SetKwBlock{Synchro}{non interruptible}{{end synchronized}}
  \SetKwFor{Foreach}{for each}{do}{endfor}
  \SetKwProg{Fn}{Function}{\string:}{}
  \SetKwProg{Proc}{Procedure}{\string:}{}
  \SetKwProg{Event}{Event}{\string:}{}
  \SetKwComment{tcp}{}{}%
  \SetKwComment{tcc}{// }{}%

  \DontPrintSemicolon
  \SetInd{0.55em}{0.55em}
  \caption{\textit{NestedLoopIterator}: a preemptable join operator used by \sagee}
  \label{algo:bgp_iterator}

  \Data{
    $tp_i$: the triple pattern to evaluate,
    $\mathcal{D}$: RDF dataset queried,
    $I_{i-1}$: iterator responsible for the evaluation of $tp_{i-1}$.
  }

  \setlength\columnsep{0pt}
  \begin{multicols*}{2}

  \Fn{Open()}{
    $I_{i-1}.Open()$ \;
    $\mu_c \leftarrow NoResult$ \;
    $I_{find} \leftarrow$ \emph{ nil; %TripleIterator} over\\an empty set of triples\;
  }

  \Fn{GetNext()}{
    \While{$I_{find}$ has read all results}{ \label{algo:line:start_outer}
      $\mu_c \leftarrow I_{i-1}.GetNext()$ \; \label{algo:line:pull_mappings}
      \If{$\mu_c = NoResult$}{
        \Return $NoResult$ \;
      }
      $I_{find} \leftarrow$ \emph{TripleIterator} over\\
      $\mu_c\llbracket tp_i \rrbracket$ in $\mathcal{D}$\; \label{algo:line:get_cursor} \label{algo:line:outer_end}
    }
    \Synchro{ \label{algo:line:start_synchro}
      \textbf{let} $\mu \leftarrow I_{find}.GetNext()$ \;
      \Return $\mu \medcup \mu_c$ \; \label{algo:line:pull_boundpattern}
    }
  }

  \Fn{Close()}{
    $I_{i-1}.Close()$ \;
  }

  \BlankLine
  \vfill
  \columnbreak

  \Fn{Stop()}{
    \textbf{Wait} until all \textbf{non interruptible} sections
    have been evaluated \;
    \textbf{Interrupt} ongoing $GetNext()$ calls \;
  }

  \Fn{Save()}{
    \textbf{let} $n \leftarrow$ the number of triples already read by $I_{find}$ \;
    \Return $\langle tp_i, \mu_c, t, n \rangle$ \;
  }

  \Fn{Load($tp', \mu', t', n$)}{
    $tp_i \leftarrow tp'$ \;
    $t \leftarrow t'$ \;
    \If{$\mu' \neq NoResult$}{
      $\mu_c \leftarrow \mu'$ \;
      $I_{find} \leftarrow$ \emph{TripleIterator} over\\
      $\mu_c\llbracket tp_i \rrbracket$ in $\mathcal{D}$\;
      \If{$n > 0$}{
        \textbf{Skip} the $n$ first results of $I_{find}$\; \label{algo:line:offset}
      }
    }
  }
\end{multicols*}
  \BlankLine
  \BlankLine
\end{algorithm}


==> figures/client_processing.tex <==
\begin{algorithm}
  \SetAlgoVlined
  \SetKwInput{KwInit}{Init}
  \SetKwFor{Foreach}{for each}{do}{endfor}
  \SetKwProg{Fn}{Function}{\string:}{}
  \SetKwProg{Proc}{Procedure}{\string:}{}
  \SetKwProg{Event}{Event}{\string:}{}
  \SetKwComment{tcp}{}{}%
  \SetKwComment{tcc}{// }{}%

  \DontPrintSemicolon
  \SetInd{0.55em}{0.55em}
  \caption{Client-side query evaluation}
  \label{algo:client_query_evaluation}

  \KwIn{
    $Q$: a BGP SPARQL query,
    $u$: url of the server
  }

  \Fn{ProcessQuery($Q$, $u$)}{
    $\mathcal{M} \leftarrow \emptyset$ \;
    $\langle \mathcal{V}, Q' \rangle \leftarrow$ send $Q$ at $u$ \;
    \While{$Q' \neq nil$}{
      $\mathcal{M} \leftarrow \mathcal{M} \medcup \mathcal{V}$; \;
      $\langle \mathcal{V}, Q' \rangle \leftarrow$ send $Q'$ at $u$ \;
    }
    \Return $\mathcal{M}$ \;
  }
  \BlankLine
\end{algorithm}


==> figures/page.tex <==
{"bindings": [{
 "?v0": ".../Offer79386",
 "?v1": ".../Product10014",
 "?v3": "\"5960\""},{
 "?v0": ".../Offer81506",
 "?v1": ".../Product10066",
 "?v3": "\"6563\"" }],
 "cardinality": 2,
"next": {
 "inner": {
  "obj":".../Country9",
  "pre":".../eligibleRegion",
  "sub":"?v0"},
  "mappings": null,
  "offset": 0,
 "source": {
   "inner": {
   "obj": "?v1",
   "pre": ".../includes",
   "sub": "?v0"},
   "mappings": {
    "?v1": ".../Product11972",
    "?v3": "\"4356\""},
   "offset": 2,
   "source": {
    "offset": 224,
    "triple": {
     "obj": "?v3",
     "pre": ".../contentSize",
     "sub": "?v1"},
     "type": "ScanIterator"},
   "type": "NestedLoopJoinIterator"},
 "type": "NestedLoopJoinIterator"}}

==> figures/plans/logical_plan.tex <==
\tikzstyle{level 1}=[level distance=0.7cm, sibling distance=1.3cm]
\begin{tikzpicture}[scale=1, transform shape, baseline=-43]
  \node {$\Pi$}
  	child {
  		node {$\bowtie$}
  			child { node {$tp_1$} }
				child { node {$tp_2$} }
	};
\end{tikzpicture}


==> figures/plans/physical_plan.tex <==
\tikzstyle{level 1}=[level distance=0.7cm, sibling distance=1.3cm]
\begin{tikzpicture}[scale=1, transform shape, baseline=-43]
  \node {$\Pi$}
  	child {
  		node {$\bowtie_{NLJ}$}
  			child { node {$tp_1$} }
				child { node {$tp_2$} }
	};
\end{tikzpicture}


==> figures/preemptable_iterator.tex <==
\begin{algorithm}
  \SetAlgoVlined
  \SetKwInput{KwInit}{Init}
  \SetKwBlock{Synchro}{synchronized}{{end synchronized}}
  \SetKwFor{Foreach}{for each}{do}{endfor}
  \SetKwProg{Fn}{Function}{\string:}{}
  \SetKwProg{Proc}{Procedure}{\string:}{}
  \SetKwProg{Event}{Event}{\string:}{}
  \SetKwComment{tcp}{}{}%
  \SetKwComment{tcc}{// }{}%

  \DontPrintSemicolon
  \SetInd{0.55em}{0.55em}
  \caption{Operations of a \textit{TripleIterator} to support preemption}
  \label{algo:preemptable_iterator}

  \Fn{TripleIterator.Stop()}{
    \textbf{Wait} until all \textbf{synchronized} sections
    have been evaluated \;
    \textbf{Interrupt} all ongoing $GetNext()$ calls \;
  }

  \Fn{TripleIterator.Save()}{
    \textbf{let} $n \leftarrow$ number of solutions already read by $C$ \;
    \Return $\langle tp, \mu_{current}, n \rangle$ \;
  }

  \Fn{TripleIterator.Load($tp', \mu', n$)}{
    $tp \leftarrow tp'$ \;
    \If{$\mu' \neq NoResult$}{
      $\mu_{current} \leftarrow \mu'$ \;
      $C \leftarrow$ a cursor over solution mappings
      for $\mu_{current}\llbracket tp \rrbracket$ in $\mathcal{D}$\;
      \If{$n > 0$}{
        \textbf{Advance} $C$ in position $n$ \;
      }
    }
  }
  \BlankLine
\end{algorithm}


==> figures/preemptable_scan.tex <==
\begin{algorithm}
  \SetKwProg{RestrictedFn}{Restricted Function}{\string:}{{end restricted}}
  \SetKwInput{KwInit}{Init}
  \SetKwFor{Foreach}{for each}{do}{endfor}
  \SetKwProg{Fn}{Function}{\string:}{end}
  \SetKwProg{Event}{Event}{\string:}{}
  \SetKwComment{tcp}{}{}%
  \SetKwComment{tcc}{// }{}%

  \DontPrintSemicolon
  \SetInd{0.55em}{0.55em}
  \caption{High-level implementation of a preemptable Scan operator}\label{algo:query_optimizer}

  \KwIn{
    $tp$: triple pattern,
    $C_{tp}$: cursor over solution mappings of $tp$ in a RDF dataset,
    $mode$: either \textsc{running} or \textsc{stopped}.
  }

  \KwInit{$\texttt{self.}mode \leftarrow$ \textsc{running}; $\texttt{self.}n \leftarrow 0$}

  \setlength\multicolsep{0pt}
  \begin{multicols*}{2}
    \RestrictedFn{Scan.Next()}{
      \If{$\texttt{self.}mode = \textsc{stopped}$}{
        \Return nil \;
      }
      $\mu \leftarrow$ advance $\texttt{self.}C_{tp}$ to find the next set of solution mappings \;
      $\texttt{self.}n \leftarrow \texttt{self.}n + 1$ \;
      \Return $\mu$ \;
    }

    \Fn{Scan.Save()} {
      \Return $\langle \texttt{self.}tp, \texttt{self.}n \rangle$ \;
    }

    \tcp*{~}
    \vfill
    \columnbreak

    \Fn{Scan.Stop()}{
      \textbf{Wait} until no restricted function is running \;
      $\texttt{self.}mode \leftarrow \textsc{stopped}$
    }

    \Fn{Scan.Load($tp'$, $n'$)}{
      $\texttt{self.}tp \leftarrow tp'$ \;
      $\texttt{self.}n \leftarrow n'$ \;
      ApplyOffset($C_{tp}$, $n$) \;
    }
  \end{multicols*}
\end{algorithm}


==> figures/q1_logical.tex <==
\begin{tikzpicture}
  \tikzstyle{level 1}=[sibling distance=2cm]
  \node (root ){$\bowtie_2$}
  child {
    node (nlj) {$\bowtie_1$}
    child { node [align=center]{$tp_2$}}
    child { node [align=center]{$tp_1$}}
  }
  child { node [align=center]{$tp_3$}};
  \end{tikzpicture}


==> figures/query_optimizer.tex <==
\begin{algorithm}
  \SetAlgoVlined
  \SetKwInput{KwInit}{Init}
  \SetKwFor{Foreach}{for each}{do}{endfor}
  \SetKwProg{Fn}{Function}{\string:}{}
  \SetKwProg{Proc}{Procedure}{\string:}{}
  \SetKwProg{Event}{Event}{\string:}{}
  \SetKwComment{tcp}{}{}%
  \SetKwComment{tcc}{// }{}%

  \DontPrintSemicolon
  \SetInd{0.55em}{0.55em}
  \caption{\sagee query optimizer}\label{algo:query_optimizer}

  \KwIn{
    $BGP = \{ tp_1, \dots, tp_n \}$: set of triples patterns,
    $\mathcal{D}$: RDF dataset queried
  }

  \Fn{BuildQueryPlan(BGP, $\mathcal{D}$)}{
    \For{$tp_i \in BGP$}{
      $tp_i.count \leftarrow cardinality(tp_i)$ \; \label{algo:line:get_cards}
    }
    \textbf{let} $BGP' \leftarrow $ \textbf{Order} $BGP$ such as $\forall tp_i \in BGP', tp_i.count \leq tp_{i+1}.count$ \; \label{algo:line:join_ordering}

    \textbf{let} $p \leftarrow TriplePatternIterator(BGP'.GetFirst(), \mathcal{D}, nil)$\; \label{algo:line:start_tree}
    remove the first triple pattern of $BGP'$\;
    \textbf{let} $\upsilon \leftarrow vars(tp)$ \;
    \While{$|BGP'| > 0$}{
      % \tcc{Search for a pattern connected to the subtree}
      \For{$tp' \in BGP'$}{
        \If{$\upsilon \cap vars(tp') \neq \emptyset$}{
          $p \leftarrow TriplePatternIterator(tp', \mathcal{D}, p)$ \;
          $\upsilon \leftarrow \upsilon \cup vars(tp')$ \;
          $BGP' \leftarrow BGP' - \{ tp' \}$ \;
        }
      }
      \Return $EmptyIterator$ \textbf{if} no connected pattern found previously \;
    }\label{algo:line:end_tree}
    \Return $p$ \;
  }
  \BlankLine
\end{algorithm}


==> figures/server_processing.tex <==
\begin{algorithm}
  \SetAlgoVlined
  \SetKwInput{KwInit}{Init}
  \SetKwFor{Foreach}{for each}{do}{endfor}
  \SetKwProg{Fn}{Function}{\string:}{}
  \SetKwProg{Proc}{Procedure}{\string:}{}
  \SetKwProg{Event}{Event}{\string:}{}
  \SetKwComment{tcp}{}{}%
  \SetKwComment{tcc}{// }{}%

  \DontPrintSemicolon
  \SetInd{0.55em}{0.55em}
  \caption{Client-side query evaluation in the Stop-and-Go query execution model}
  \label{algo:server_query_evaluation}

  \KwIn{
    $Q$: a server-specific query,
    $\mathcal{D}$: RDF dataset,
    $q$: quota in time
  }

  \Fn{EvaluateQuery($Q$, $\mathcal{D}$, $q$)}{
    \eIf{$Q$ is a saved query execution plan}{
      $P \leftarrow Reload(Q)$ \; \label{algo:line:reload_query}
    }{
      $P \leftarrow BuildQueryPlan(Q, \mathcal{D})$ \; \label{algo:line:build_query_plan}
    }

    \tcc{Evaluate the query execution plan under the time quota}
    $\mathcal{V} \leftarrow \emptyset$ \;
    \textbf{Start Timer} invoke $P.Stop()$ after $q$ is exceeded \; \label{algo:line:start_timer}
    \While{\textbf{not} $P.IsDone()$}{ \label{algo:line:plan_evaluation}
      $\mu \leftarrow P.Next()$ \; \label{algo:line:advance_plan}
      $\mathcal{V} \leftarrow \mathcal{V} \medcup \{ \mu \}$ \;
    }

    \tcc{Save query execution plan for the next evaluation step}
    $Q' \leftarrow nil$ \;
    \If{\textbf{not} $P.IsDone()$}{
      $Q' \leftarrow P.Save()$ \; \label{algo:line:serialize_plan}
    }
    \Return $\langle \mathcal{V}, Q' \rangle$ \;
  }
  \BlankLine
\end{algorithm}

